Dynamical mean-field theory from a quantum chemical perspective

We investigate the dynamical mean-field theory (DMFT) from a quantum chemical perspective. Dynamical mean-field theory offers a formalism to extend quantum chemical methods for finite systems to infinite periodic problems within a local correlation approximation. In addition, quantum chemical techniques can be used to construct new ab-initio Hamiltonians and impurity solvers for DMFT. Here we explore some ways in which these things may be achieved. First, we present an informal overview of dynamical mean-field theory to connect to quantum chemical language. Next we describe an implementation of dynamical mean-field theory where we start from an ab-initio Hartree- Fock Hamiltonian that avoids double counting issues present in many applications of DMFT. We then explore the use of the configuration interaction hierarchy in DMFT as an approximate solver for the impurity problem. We also investigate some numerical issues of convergence within DMFT. Our studies are carried out in the context of the cubic hydrogen model, a simple but challenging test for correlation methods. Finally we finish with some conclusions for future directions.

==> algorithm.tex <==
\section{DMFT algorithm}

%% make note about self-consistency and open particle number.

We now  summarize the DMFT algorithm in our implementation that follows the basic ideas outlined in the previous section.
Within the Hamiltonian formulation we can view the DMFT local Green's function
as a function of three variables $N$ (particle number of the impurity model), $\mu$ (chemical potential), and the local self-energy
$\mathbf{\Sigma}(\omega)$. All three have to be solved for together. At the solution point of the DMFT algorithm, $N$ minimises
 the ground-state energy of the impurity model $E(N, \mu, \mathbf{\Sigma})$, $\mu$ yields
the correct particle number of the crystal, and $\mathbf{\Sigma}(\omega)$ satisfies the DMFT
self-consistency conditions (\ref{eq:self_e_scheme}), (\ref{eq:hybrid_scheme}). We thus arrange our algorithm in three loops
\begin{enumerate}
\item Search over particle number $N$ to be used in the impurity model,
\item For each $N$, search over chemical potential $\mu$ to satisfy the total crystal particle number constraint,
\item For each $N, \mu$, iterate the DMFT self-consistency equations.
\end{enumerate}
Step 1 below corresponds to the initialisation of the DMFT procedure, while steps 2-8 constitute the  loops described above.
\begin{enumerate}
\item Search over $N$ in impurity model
\begin{enumerate}
\item Search over $\mu$. 
\end{enumerate}
\end{enumerate}

%% \item \textit{Initialisation} 
%%   We perform a Hartree-Fock (HF) calculation on the crystal 
%% in a local basis. From the HF calculation we extract the following quantities
%%  in the computational unit cell: the Fock matrix $\mathbf{F}(\mathbf{k})$ and 
%% overlap matrix $\mathbf{S}(\mathbf{k})$ in  $k$-space, and the Hartree-Fock density matrix 
%% $\mathbf{P}(\mathbf{R}_0)$ in  real space. 
%% \item \textit{Loop over N, $\mu$}. For each $N



%% To determine $N$ we minimize the ground-state energy of the impurity model $E(N, \mu, \mathbf{\Sigma}(\omega)$

%% $ \mu, \mathbf{\Sigma}(\omega)$, that are determined by the DMFT algorithm.
%% the following parameters
%% These are
%% \begin{itemize}
%% \item A loop over the  particle number $N$ of the impurity problem, to search for the $N$ which
%% yields the lowest energy ground-state of the impurity problem.
%% \item A loop over the chemical potential $\mu$ to satisfy the crystal particle number constraint.
%% \item A self-consistency loop for the given $N, \mu$ to satisfy the DMFT self-consistency conditions (\ref{eq:self_e_scheme}), (\ref{eq:hybrid_scheme}).
%% \end{itemize}


%% The steps $2-8$ listed below are performed inside a loop that enables us to perform
%% a search over all values of the possible chemical potential $\mu$ in order to choose one that gives a proper number of electrons in the unit cell. 
%% The number of electrons $N$ that minimizes the energy is found at step~$4$ described bellow. 
%% The detailed  aspects of each part of the algorithm,
%% such as  bath construction, the solver, and  self-consistency, are discussed   in sections Sec. \ref{sec:bath}, \ref{sec:solver},
%% \ref{sec:consistency}. We recall from above that our intent is to construct an \textit{ab-initio} 
%% formulation of DMFT free from the uncontrolled approximations in DFT-DMFT. Thus, we design it to follow a similar scheme, 
%% first Hartree-Fock calculation and then a correlated calculation on the system of interest, as one 
%%  would ordinarily design calculations using molecular systems. 
%% \begin{enumerate}
%% \item \textit{Initialisation}. 

\begin{enumerate}

\item \textbf{Impurity model particle number search}. Search over particle number $N$ in the impurity problem to
find $N$ corresponding to the lowest ground-state energy of the impurity Hamiltonian. 

\item \textbf{Chemical potential search}


and $\mu$ to find the $N$ which yields
the lowest energy self-consistent ground-state of the impurity model and the $\mu$ which yields the crystal particle number constraint.
For each $N$ and $\mu$, 

%% \item % We adjust the chemical potential $\mu$ so that the number of electrons in the unit cell is
%% %correct, using the integration formula
%% %\begin{align}
%% %\end{align}
%% We calculate the of number of electrons in the unit cell by integrating on the imaginary axis 
%%  the Green's function from the Eq.~(\ref{eq:dmft_local_greens}) that was constructed for the newly obtained self-energy. 
%% The details of the numerical integration are studied in  section X.  


\item \textit{Construction of the impurity Hamiltonian}. $\mathbf{F}(\mathbf{k})$ and  $\mathbf{S}({\mathbf{k}})$ are 
used to construct the one-body impurity Hamiltonian  $\mathbf{F}$
and overlap matrix $\mathbf{S}$ with corrections for non-orthogonality,
according to Eq.~(\ref{eq:savrasov_hamiltonian}) and Eq.~(\ref{eq:savrasov_overlap}) respectively.
%% These include
%% the non-orthogonality corrections 
%% as described in section \ref{sec:hamiltonian}.
%% unit cell in the real space. 
%% Such a Hamiltonian is not just a simple Fourier transform of the k-space Fock matrix, 
%% $\mathbf{F}_{k}$,  
%% due to the non-orthogonality of the orbital basis, and consequently the 1-body Hamiltonian $\mathbf{F}$ must be constructed as described 
%% in Sec.~\ref{sec:savrasov_correction}. 
The  2-body integrals $w_{ijkl}$ are  computed in the  
same local basis of the computational unit cell as used
for the crystal calculation. Finally, the Hartree-Fock mean-field contribution from the unit cell is removed as described in section \ref{sec:hamiltonian}, giving a final impurity one-electron Hamiltonian
\begin{align}
\tilde{F}_{i j} =F_{i j}-\sum_{k l \in  {\rm act}}P^{HF}_{k l} (w_{ijlk} - \frac{1}{2} w_{iklj})
\end{align}
%%((i j|l k)-0.5(i k|l j)),
where the indices $i$, $j$, $k$, and $l$ run only within the (active space) of the unit cell and the density matrix $\mathbf{P}$ 
for the active orbitals is obtained from $\mathbf{P}(\mathbf{R}_0)$ in the HF calculation. 

%% (We use the same Gaussian basis as used in the crystal calculation).
%% \item construct the impurity Hamiltonian with the Hartree-Fock mean-field unit-cell terms removed For a molecular calculation one would only use the kinetic and nuclear-electron part of the Hamiltonian to build the 1-body part of 
%% the full Hamiltonian.
%% The part that comes from multiplying the 2-body integrals by density matrix would be not included since this contribution will be calculated again 
%% in the correlated calculation. Similarly, here we have to subtract this contribution for the unit cell of interest

\item \textit{Bath construction}. We obtain the parameters of the bath Hamiltonian, $\epsilon_{p}$ and $V_{p i}$  by least-squares fitting the non-interacting bath expression (\ref{eq:bath_representation}) to the hybridization $\mathbf{\Delta}(\omega)$ defined on a set of imaginary frequencies, as
\begin{align}
\mathbf{\Delta}(i\omega) = (i\omega + \mu)\mathbf{S} - \tilde{\mathbf{F}} - \mathbf{G}^{-1}(\mathbf{R}_0, i\omega) - \mathbf{\Sigma}(i\omega) \label{eq:hybrid}
\end{align}
In the first iteration, we take $\mathbf{\Delta}(i\omega)$ to be the Hartree-Fock hybridization. This corresponds to $\mathbf{\Sigma}(i\omega) = 0$ in the 
 $\mathbf{G}(\mathbf{R}_0,i\omega)$ formula.
%% From the Hartree-Fock Green's function, 
%%  by fitting
%% the Hartree-Fock hybFor a set of imaginary frequencies ${i\omega}$ the lattice Green's from the k-space calculation 
%% on the whole crystalline system 
%% \begin{equation}
%%  \mathbf{ G}(i\omega)=\sum_{k}\frac{1}{(i\omega+\mu)\mathbf{S}_{k}-\mathbf{ F}_{k}-\mathbf{ \Sigma}(i\omega)} \label{eq:lattice_G}
%% \end{equation}
%% is mapped onto a real space local Green's function of a unit cell embedded in a bath 
%% \begin{equation}
%%  \mathbf{ G}_{\rm loc}(i\omega)=\frac{1}{(i\omega+\mu)\mathbf{S}-\mathbf{F}-\mathbf{\Delta}(i\omega)-\mathbf{\Sigma}(i\omega)},
%% \end{equation}
%% where $\mathbf{F}$ and $\mathbf{S}$ are Fock and overlap matrix in the real space constructed according to Eq.~\ref{eq:savrasov_fock} and 
%% Eq.~\ref{eq:savrasov_overlap}, respectively. The self-energy, $\mathbf{\Sigma}(i\omega)$, is zero  
%% within the first DMFT iteration since $\mathbf{ G}(i\omega)$ is a HF Green's function.  
%% Subsequently, the $\omega$--dependent hybridization $\Delta(i\omega)_{ij}$ is calculated from 
%% \begin{equation}
%% \mathbf{\Delta}(i\omega)=(i\omega+\mu)\mathbf{S}-\mathbf{F}-\mathbf{ G}(i\omega)-\mathbf{\Sigma}(i\omega), \label{eq:delta_from_G}
%% \end{equation}  
%% \begin{equation}
%% \Delta(i\omega)_{ij}=\sum_{\kappa}\frac{V_{i\kappa}V_{\kappa j}}{i\omega - \epsilon_{\kappa}}. \label{eq:hybridization_v_sps}
%% \end{equation}  
Further technical details of the bath fitting procedure are described in  section \ref{sec:fitting}.
\item \textit{Calculation of the impurity Greens function}. 
For the given $N$, we calculate the ground-state
wavefunction of the impurity problem Hamiltonian. 
%% First, we search for the ground-state wave function for given $\mu$, which requires searching over all possible electron
%% numbers contained in the impurity problem within the given wave function approximation. 
For a set of imaginary frequencies, we next calculate the impurity Green's function. We describe
the calculation of the wavefucntion and Green's function based on the Restricted Active Space Configuration Interaction (RASCI) method, in
section \ref{sec:rasci}.
%% Having obtained the 1-body Hamiltonian $\mathbf{\tilde{F}}$ and the 2-body integrals $v_{ijkl}$, one searches for ground state wave function 
%% and corresponding number of electrons by performing a search over the possible electron numbers contained in the unit cell and the bath.
%% The obtained $|\Psi_{0}\rangle$ is used for calculating the unit cell Green's function $\mathbf{G}_{imp}(i\omega)$ from the expression
%% \begin{equation}
%% Here \ should  \ be \ just \ a \ reference \ to \ Garnet's \ equation 
%% \end{equation}  
%% where labels $i$, $j$ are the orbital indeces within the unit cell and the impurity Green's function is calculated for a set of imaginary frequencies.
%% In our particular case, 
\item 
%%Calculation of the self-energy. After the evaluation of the unit cell Green's function, $\mathbf{G}_{imp}(i\omega)$, from the solver, 
\textit{Calculation of the self-energy}. The DMFT self-energy is calculated from the Dyson equation as 
\begin{equation}
\mathbf{\Sigma}_{\rm new}(i\omega)=\mathbf{G}_{0}(i\omega)^{-1}-\mathbf{G}_{imp}(i\omega)^{-1},
\end{equation}
where $\mathbf{G}_{0}(i\omega)$ is defined as 
\begin{equation}
 \mathbf{ G}_{0}(i\omega)=\frac{1}{(i\omega+\mu)\mathbf{S}-\tilde{\mathbf{F}}-\mathbf{\Delta}(i\omega)}.
\end{equation}
\item \textit{Convergence check}. We check if the difference between the self-energy from the current and the previous iteration, 
$A=\sum_{\omega}|\sum_{ij}([\Sigma_{\rm old}(i\omega)]_{ij}-[\Sigma_{\rm new}(i\omega)]_{ij})|$, 
is below a desired threshold, $thresh$. If $A\le thresh$ then one quits the self-consistency cycle.
\item 
Come back to the point~2 and construct a new 1-body Hamiltonian according to the Eq.~\ref{eq:savrasov_hamiltonian} using the newly evaluated self-energy 
$\mathbf{\Sigma}_{\rm new}(i\omega)$. 
\end{enumerate}

During the steps of the cycle, all the quatities such as local crystal Green's function $\mathbf{G}(i\omega)$, 
impurity Green'sfunction$\mathbf{G}_{imp}(i\omega)$ and the self-energy
$\mathbf{\Sigma}(i\omega)$ due to the smoothnes of the Green's function are calculated for a set of imaginary frequencies. 
  


==> results.tex <==
%% \documentclass[letterpaper, 12pt]{revtex4}
%% \usepackage{amsmath}
%% \usepackage{graphicx}
%% \usepackage{dcolumn}
%%\begin{document}
\section{DMFT algorithm}

%% make note about self-consistency and open particle number.

We now  summarize the DMFT algorithm in our implementation, following the basic ideas outlined in the previous section.
The steps $2-8$ listed below are performed inside two loops that enable us to perform
{\bf (i)} a search for the ground state over all possible number of electrons contained in the impurity model in order to find 
a number of electrons $N$ that minimizes the energy
{\bf (ii)} a search 
over all the possible values of chemical potential $\mu$ in order to choose one that gives a proper number of electrons in the unit cell $n_{UC}$. 

%% The detailed  aspects of each part of the algorithm,
%% such as  bath construction, the solver, and  self-consistency, are discussed   in sections Sec. \ref{sec:bath}, \ref{sec:solver},
%% \ref{sec:consistency}. We recall from above that our intent is to construct an \textit{ab-initio} 
%% formulation of DMFT free from the uncontrolled approximations in DFT-DMFT. Thus, we design it to follow a similar scheme, 
%% first Hartree-Fock calculation and then a correlated calculation on the system of interest, as one 
%%  would ordinarily design calculations using molecular systems. 
\begin{enumerate}
\item We perform a Hartree-Fock (HF) calculation on the crystal 
in a local basis.
From the HF calculation we extract the following quantities
 in the computational unit cell: 
the Fock matrix $\mathbf{F}(\mathbf{k})$ and 
overlap matrix $\mathbf{S}(\mathbf{k})$ in  $k$-space, and the 
Hartree-Fock density matrix 
$\mathbf{P}(\mathbf{R}_0)$ in  real space. 
\item  $\mathbf{F}(\mathbf{k})$ and  $\mathbf{S}({\mathbf{k}})$ are 
used to construct the one-body Hamiltonian  $\mathbf{F}$
and overlap matrix $\mathbf{S}$ 
of the impurity problem, 
according to Eq.~(\ref{eq:savrasov_hamiltonian}) and Eq.~(\ref{eq:savrasov_overlap}) respectively.
These include
the non-orthogonality corrections 
as described in section \ref{sec:hamiltonian}.
%% unit cell in the real space. 
%% Such a Hamiltonian is not just a simple Fourier transform of the k-space Fock matrix, 
%% $\mathbf{F}_{k}$,  
%% due to the non-orthogonality of the orbital basis, and consequently the 1-body Hamiltonian $\mathbf{F}$ must be constructed as described 
%% in Sec.~\ref{sec:savrasov_correction}. 
The  2-body integrals $w_{ijkl}$ are  computed in the  
same local basis of the computational unit cell as used
for the crystal calculation. Finally, the Hartree-Fock mean-field contribution from the unit cell is removed as described in section \ref{sec:hamiltonian}, giving a final unit cell one-electron Hamiltonian (in the unit-cell orbitals)
\begin{align}
\tilde{F}_{i j} =F_{i j}-\sum_{k l \in  {\rm act}}P^{HF}_{k l} (w_{ijlk} - \frac{1}{2} w_{iklj})
\end{align}
%%((i j|l k)-0.5(i k|l j)),
where the indices $i$, $j$, $k$, and $l$ run only within the (active space) of the unit cell and the density matrix $\mathbf{P}$ 
for the active orbitals is obtained from $\mathbf{P}(\mathbf{R}_0)$ in the HF calculation. 

%% (We use the same Gaussian basis as used in the crystal calculation).
%% \item construct the impurity Hamiltonian with the Hartree-Fock mean-field unit-cell terms removed For a molecular calculation one would only use the kinetic and nuclear-electron part of the Hamiltonian to build the 1-body part of 
%% the full Hamiltonian.
%% The part that comes from multiplying the 2-body integrals by density matrix would be not included since this contribution will be calculated again 
%% in the correlated calculation. Similarly, here we have to subtract this contribution for the unit cell of interest

\item We obtain bath parameters $\epsilon_{\kappa}$ and $V_{\kappa i}$ for the impurity problem by least-squares fitting the non-interacting bath expression (\ref{eq:bath_representation}) to the hybridization $\mathbf{\Delta}(\omega)$ defined on a set of imaginary frequencies as
\begin{align}
\mathbf{\Delta}(i\omega) = (i\omega + \mu)\mathbf{S} - \tilde{\mathbf{F}} - \mathbf{G}^{-1}(\mathbf{R}_0, i\omega) - \mathbf{\Sigma}(i\omega) \label{eq:hybrid}
\end{align}
In the first iteration, we take $\mathbf{\Delta}(i\omega)$ to be the Hartree-Fock hybridization. This corresponds to $\mathbf{\Sigma}(i\omega) = 0$ in the 
 $\mathbf{G}(\mathbf{R}_0,i\omega)$ formula.
%% From the Hartree-Fock Green's function, 
%%  by fitting
%% the Hartree-Fock hybFor a set of imaginary frequencies ${i\omega}$ the lattice Green's from the k-space calculation 
%% on the whole crystalline system 
%% \begin{equation}
%%  \mathbf{ G}(i\omega)=\sum_{k}\frac{1}{(i\omega+\mu)\mathbf{S}_{k}-\mathbf{ F}_{k}-\mathbf{ \Sigma}(i\omega)} \label{eq:lattice_G}
%% \end{equation}
%% is mapped onto a real space local Green's function of a unit cell embedded in a bath 
%% \begin{equation}
%%  \mathbf{ G}_{\rm loc}(i\omega)=\frac{1}{(i\omega+\mu)\mathbf{S}-\mathbf{F}-\mathbf{\Delta}(i\omega)-\mathbf{\Sigma}(i\omega)},
%% \end{equation}
%% where $\mathbf{F}$ and $\mathbf{S}$ are Fock and overlap matrix in the real space constructed according to Eq.~\ref{eq:savrasov_fock} and 
%% Eq.~\ref{eq:savrasov_overlap}, respectively. The self-energy, $\mathbf{\Sigma}(i\omega)$, is zero  
%% within the first DMFT iteration since $\mathbf{ G}(i\omega)$ is a HF Green's function.  
%% Subsequently, the $\omega$--dependent hybridization $\Delta(i\omega)_{ij}$ is calculated from 
%% \begin{equation}
%% \mathbf{\Delta}(i\omega)=(i\omega+\mu)\mathbf{S}-\mathbf{F}-\mathbf{ G}(i\omega)-\mathbf{\Sigma}(i\omega), \label{eq:delta_from_G}
%% \end{equation}  
%% \begin{equation}
%% \Delta(i\omega)_{ij}=\sum_{\kappa}\frac{V_{i\kappa}V_{\kappa j}}{i\omega - \epsilon_{\kappa}}. \label{eq:hybridization_v_sps}
%% \end{equation}  
Further technical details of the bath fitting procedure are described in  section \ref{sec:fitting}.
\item
First, the ground state wave function $|\Psi_{0}\rangle$ is calculated for given $\mu$ and $N$. 
Next, for a set of imaginary frequencies, using the earlier calculated wave function $|\Psi_{0}\rangle$, we calculate the impurity Green's function 
using a quantum chemistry wave function-based solver. 
We describe the calculation of the Green's function based on the Restricted Active Space Configuration Interaction (RASCI) method, 
section \ref{sec:rasci}.
%% Having obtained the 1-body Hamiltonian $\mathbf{\tilde{F}}$ and the 2-body integrals $v_{ijkl}$, one searches for ground state wave function 
%% and corresponding number of electrons by performing a search over the possible electron numbers contained in the unit cell and the bath.
%% The obtained $|\Psi_{0}\rangle$ is used for calculating the unit cell Green's function $\mathbf{G}_{imp}(i\omega)$ from the expression
%% \begin{equation}
%% Here \ should  \ be \ just \ a \ reference \ to \ Garnet's \ equation 
%% \end{equation}  
%% where labels $i$, $j$ are the orbital indeces within the unit cell and the impurity Green's function is calculated for a set of imaginary frequencies.
%% In our particular case, 
\item 
%%Calculation of the self-energy. After the evaluation of the unit cell Green's function, $\mathbf{G}_{imp}(i\omega)$, from the solver, 
The DMFT self-energy is calculated from the Dyson equation as 
\begin{equation}
\mathbf{\Sigma}_{\rm new}(i\omega)=\mathbf{G}_{0}(i\omega)^{-1}-\mathbf{G}_{imp}(i\omega)^{-1},
\end{equation}
where $\mathbf{G}_{0}(i\omega)$ is defined as 
\begin{equation}
 \mathbf{ G}_{0}(i\omega)=\frac{1}{(i\omega+\mu)\mathbf{S}-\tilde{\mathbf{F}}-\mathbf{\Delta}(i\omega)}.
\end{equation}
\item We check if the difference between the self-energy from the current and the previous iteration, 
$A=\sum_{\omega}|\sum_{ij}([\Sigma_{\rm old}(i\omega)]_{ij}-[\Sigma_{\rm new}(i\omega)]_{ij})|$, 
is below a desired threshold, $thresh$. If $A\le thresh$ then one quits the self-consistency cycle.
\item % We adjust the chemical potential $\mu$ so that the number of electrons in the unit cell is
%correct, using the integration formula
%\begin{align}
%\end{align}
We calculate the of number of electrons in the unit cell by integrating on the imaginary axis 
 the Green's function from the Eq.~(\ref{eq:dmft_local_greens}) that was constructed for the newly obtained self-energy. 
The details of the numerical integration are studied in  section X.  
\item 
Come back to the point~2 and construct a new 1-body Hamiltonian according to the Eq.~(\ref{eq:savrasov_hamiltonian}) using the newly evaluated self-energy 
$\mathbf{\Sigma}_{\rm new}(i\omega)$. 
\end{enumerate}

During the steps of the cycle, all the quantities such as local crystal Green's function $\mathbf{G}(i\omega)$, 
impurity Green's function $\mathbf{G}_{imp}(i\omega)$, and the self-energy
$\mathbf{\Sigma}(i\omega)$ due to the smoothness of the Green's function are calculated for a set of imaginary frequencies. 
  


